High Mass Inner Regions Found in Five Outbursting Sources

Young stellar objects are thought to commonly undergo sudden accretion events that result in a rise in bolometric luminosity. These outbursts likely coincide with the onset of planet formation, and could impact the formation of planets. The reason behind this dramatic enhancement of accretion is an active area of research, and the mass of the system is a critical parameter. Using Northern Extended Millimeter Array, we survey five outbursting sources (three FU Ori, one EX Or, one 'peculiar' source) with the primary goal of determining the system's mass using an optically thin line of CO. We estimate the mass of a central region for each object that using both continuum emission and C17O J=2-1. The C17O emission likely includes both disk and inner envelope material, thus acts as an upper limit on the disk mass, ranging from 0.33-3.4 Msun for our sources. These derived masses suggest that the inner approx. 1000 au contains enough mass along the line of sight for these sources to be gravitationally unstable.

==> molecular_tables.tex <==
\begin{deluxetable*}{cccccccc}
\label{tab:Common lines}
\tablecolumns{7}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{Identified Lines Across all Outburst Sources}
\tablehead{Molecule	&	Transition	&	Frequency (GHz)	& V1057 Cyg &	V1515 Cyg	&	V1647 Ori	&	V1735 Cyg	&	V2492 Cyg}
\startdata
\ce{^{13}CO}	&	J=2-1	&	220.399	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{C^{18}O}	&	J=2-1	&	219.560	& yes&	yes	&	yes	&	yes	&	yes	\\
\ce{C^{17}O}	&	J=2-1	&	224.714	& yes&	yes	&	yes	&	yes	&	yes	\\
SO	&	4(5)- 3(4)	&	206.176	& yes&	yes	&	yes	&	yes	&	yes	\\
SO	&	6(5)-5(4)	&	219.949	& yes&	yes	&	yes	&	yes	&	yes	\\
\ce{SO2}	&	12(0,12)-11(1,11)	&	203.392	& yes &	maybe	&		&		&		\\
\ce{SO2}	&	11(2,10)- 11(1,11)	 &	205.301	& yes  &		&		&	maybe	&		\\
\ce{H2CO}	&	3(0,3)-2(0,2)	& 	218.222	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{H2CO}	&	3(1,2)-2(1,1)	&	225.698	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{H2CO}	&	3(2,2)-2(2,1)	&	218.476	& yes &		&		&	maybe	&	yes	\\
\ce{H2CO}	&	3(2,1)-2(2,0)	&	218.760	& yes &		&		&	yes	&	maybe	\\
\enddata
\tablecomments{All of the above molecules and transitions have a bright detection in source V1057 Cyg, and either have a bright detection (noted with `yes') or tentative detection (noted with `maybe') in each corresponding source. }
\end{deluxetable*}

\colorlet{color1}{green!10!white}
\colorlet{color2}{cyan!10!white}
\colorlet{color3}{red!10!white}
\colorlet{color4}{olive!10!white}

\begin{deluxetable*}{ccc}
\label{tab:Bonus_lines}
\tablecolumns{3}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{Additional Identified Lines In V1057 Cyg}
\tablehead{Molecule	&	Transition	&	Frequency (GHz)}
\startdata
\rowcolor{color1} \multicolumn{3}{c}{Carbon Isotopologue}\\
\ce{^{13}C^{18}O}	&	2-1	&	209.419	\\
\rowcolor{color2} \multicolumn{3}{c}{Water}\\			
HDO	&	3( 1, 2)- 2( 2, 1)	&	225.897	\\	
\rowcolor{color3} \multicolumn{3}{c}{Sulfur Species}\\
OCS	&	17-16	&	206.745	\\
OCS	&	18-17	&	218.903	\\
\ce{SO2}	&	3( 2, 2)- 2( 1, 1)	&	208.700	\\
\ce{SO2}	&	11( 1,11)-10( 0,10)	&	221.965	\\
\ce{SO2}	&	20( 2,18)-19( 3,17)	&	224.265	\\
\ce{SO2}	&	13( 2,12)-13( 1,13)	&	225.154	\\
\ce{H2CS}	&	6( 1, 6)- 5( 1, 5)	&	202.924	\\
\ce{H2CS}	&	6( 0, 6)- 5( 0, 5)	&	205.988	\\
\ce{H2CS}	&	6( 1, 5)- 5( 1, 4)	&	209.200	\\
\rowcolor{color4} \multicolumn{3}{c}{Building-block COMs}\\		
\ce{CH3CN }	&	12-11 k = 3	&	220.709	\\
\ce{CH3CN} 	&	12-11 k = 2	&	220.730	\\
\ce{CH3CN} 	&	12-11 k = 1	&	220.743	\\
\ce{CH3CN} 	&	12-11 k = 0	&	220.747	\\
\ce{H3CN}	&	23-22	&	209.230	\\
\ce{H3CN}	&	24-23	&	218.325	\\
\ce{H2^{13}CO}	&	3( 1, 3)- 2( 1, 2)	&	206.132	\\
\ce{H2^{13}CO}	&	3(1,2)-2(1,1)	&	219.908	\\
\ce{CH3OH}	&	1( 1) + - 2( 0) + vt=0	&	205.791	\\
\ce{CH3OH}	&	4(2,2)-3(1,2)	&	218.440	\\
\ce{CH2DOH}	&	10(1,9) - 9(1,8)	&	203.937	\\
\ce{CH2DOH}	&	7(2,6) - 7(1,7), e1	&	224.701	\\
\rowcolor{LightYellow} \multicolumn{3}{c}{Long COMs}\\			
\ce{CH3OCH3}	&	11( 1,11)-10( 0,10)	&	209.515	\\
\ce{CH3OCHO}	&	18( 6,13)- 17( 6,12) E	&	224.022	\\
\ce{CH3OCHO}	&	8( 5,14)- 17( 5,13) A	&	224.328	\\
\enddata
\tablecomments{These molecules and associated transitions show up as bright detections. There are more long COMs with tentative detections that will be used to confirm the existence of these COMs in V1057 Cyg}
\end{deluxetable*}

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{images/Line_rich_example.pdf}
    \caption{\textit{An example of the spectra of the central pixel of each source between 218.2-219 GHz. This region shows how V1057 Cyg is markedly more line-rich than each of the other sources. }}
    \label{fig:line-rich-example}
\end{figure*}
